Mask-conditioned latent diffusion for generating gastrointestinal polyp images

In order to take advantage of AI solutions in endoscopy diagnostics, we must overcome the issue of limited annotations. These limitations are caused by the high privacy concerns in the medical field and the requirement of getting aid from experts for the time-consuming and costly medical data annotation process. In computer vision, image synthesis has made a significant contribution in recent years as a result of the progress of generative adversarial networks (GANs) and diffusion probabilistic models (DPM). Novel DPMs have outperformed GANs in text, image, and video generation tasks. Therefore, this study proposes a conditional DPM framework to generate synthetic GI polyp images conditioned on given generated segmentation masks. Our experimental results show that our system can generate an unlimited number of high-fidelity synthetic polyp images with the corresponding ground truth masks of polyps. To test the usefulness of the generated data, we trained binary image segmentation models to study the effect of using synthetic data. Results show that the best micro-imagewise IOU of 0.7751 was achieved from DeepLabv3+ when the training data consists of both real data and synthetic data. However, the results reflect that achieving good segmentation performance with synthetic data heavily depends on model architectures.

==> backups/authors.tex <==
\author{\IEEEauthorblockN{Roman Macháček}
\IEEEauthorblockA{%\textit{dept. name of organization (of Aff.)} \\
\textit{University of Oslo }\\
Oslo, Norway \\
ro.machacek0@gmail.com}
\and
\IEEEauthorblockN{Leila Mozaffari}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{Oslo Metropolitan University}\\
Oslo, Norway \\
s372060@oslomet.no}
\and
\IEEEauthorblockN{Zahra Sepasdar}
\IEEEauthorblockA{\textit{Monash Biomedical Imaging} \\
\textit{Monash University}\\
Melbourne, Australia \\
zahra.sepasdar@monash.edu}
\and
\IEEEauthorblockN{Sravanthi Parasa}
\IEEEauthorblockA{\textit{Department of Gastroenterology} \\
\textit{
Swedish Medical Group}\\
Seattle, USA \\
vaidhya209@gmail.com}
\and
\IEEEauthorblockN{P{\aa}l Halvorsen}
\IEEEauthorblockA{%\textit{dept. name of organization (of Aff.)} \\
\textit{SimulaMet}\\
Oslo, Norway \\
paalh@simula.no}
\and
\IEEEauthorblockN{Michael A. Riegler}
\IEEEauthorblockA{%\textit{dept. name of organization (of Aff.)} \\
\textit{SimulaMet}\\
Oslo, Norway \\
michael@simula.no}
\and
\IEEEauthorblockN{Vajira Thambawita}
\IEEEauthorblockA{ %\textit{dept. name of organization (of Aff.)} \\
\textit{SimulaMet}\\
Oslo, Norway \\
vajira@simula.no}

}
